CarPlanner: Consistent Auto-regressive Trajectory Planning for Large-scale Reinforcement Learning in Autonomous Driving

Trajectory planning is vital for autonomous driving, ensuring safe and efficient navigation in complex environments. While recent learning-based methods, particularly reinforcement learning (RL), have shown promise in specific scenarios, RL planners struggle with training inefficiencies and managing large-scale, real-world driving scenarios. In this paper, we introduce \textbf{CarPlanner}, a \textbf{C}onsistent \textbf{a}uto-\textbf{r}egressive \textbf{Planner} that uses RL to generate multi-modal trajectories. The auto-regressive structure enables efficient large-scale RL training, while the incorporation of consistency ensures stable policy learning by maintaining coherent temporal consistency across time steps. Moreover, CarPlanner employs a generation-selection framework with an expert-guided reward function and an invariant-view module, simplifying RL training and enhancing policy performance. Extensive analysis demonstrates that our proposed RL framework effectively addresses the challenges of training efficiency and performance enhancement, positioning CarPlanner as a promising solution for trajectory planning in autonomous driving. To the best of our knowledge, we are the first to demonstrate that the RL-based planner can surpass both IL- and rule-based state-of-the-arts (SOTAs) on the challenging large-scale real-world dataset nuPlan. Our proposed CarPlanner surpasses RL-, IL-, and rule-based SOTA approaches within this demanding dataset.

==> blocks/table_supple_rl_horizon.tex <==


\begin{table}[t]
    % \vspace{6pt}
    \centering
    % \vspace{-0.2cm}
    \setlength{\tabcolsep}{3pt} % Adjust the space between columns
    \setlength{\aboverulesep}{0.3pt}
    \setlength{\belowrulesep}{0.3pt}
    % \small
    \fontsize{5pt}{6pt}\selectfont % Set font size and line spacing
    \resizebox{0.49\textwidth}{!}{\begin{tabular}{c | c |  c c c c c  }
    \toprule
    \multicolumn{2}{c|}{Time horizon} & \multicolumn{5}{c}{Closed-loop metrics ($\uparrow$)}  \\
    \midrule
    Train & \makecell{Test} &  CLS-NR &  S-CR  & S-Area  & S-PR & S-Comfort   \\
    \midrule
    \multirow{4}{*}{\makecell{1}} 
            & 1     &  75.79 & 87.18  & 88.89  & 90.99  & 87.18   \\ 
            & 3     &  73.04 & 86.70  & 92.66  & 86.33  & 63.30   \\ 
            & 5     &  71.55 & 85.91  & 91.82  & 85.69  & 60.91   \\ 
            & 8     &  71.55 & 85.91  & 91.82  & 85.69  & 60.91   \\ 
    \midrule
    \multirow{4}{*}{\makecell{3}} 
            & 1     &  86.08 & 95.95  & 97.68  & 85.70  & 84.17   \\ 
            & 3     &  88.65 & 97.10  & 97.68  & 87.96  & 92.66   \\ 
            & 5     &  89.39 & 97.31  & 98.46  & 88.04  & 86.54   \\ 
            & 8     &  89.36 & 97.31  & 98.46  & 87.93  & 86.54   \\ 
    \midrule
    \multirow{4}{*}{\makecell{5}} 
            & 1     &  85.09 & 95.56  & 96.53  & 89.92  & 89.58   \\ 
            & 3     &  91.14 & 96.73  & 98.85  & 91.95  & 91.54   \\ 
            & 5     &  91.72 & 97.69  & 98.85  & 92.58  & 90.77   \\ 
            & 8     &  91.80 & 98.08  & 98.85  & 92.55  & 90.38   \\ 
    \midrule
    \multirow{4}{*}{\makecell{8}} 
            & 1     &  87.43 & 94.98  & 98.46  & 91.13  & 90.73   \\ 
            & 3     &  93.93 & 98.84  & 98.84  & 94.97  & 91.86   \\ 
            & 5     &  93.94 & 99.22  & 99.22  & 95.04  & 91.09   \\ 
            & 8     &  94.07 & 99.22  & 99.22  & 95.06  & 91.09   \\ 
    \bottomrule
    \end{tabular}}
    % \vspace{-0.3cm}
    \caption{\red{todo}}
    \label{table:supple-abla-rl-horizon}
    % \vspace{-0.3cm}
\end{table}


